Similarity quantification for linear stochastic systems: A coupling compensator approach

For the formal verification and design of control systems, abstractions with quantified accuracy are crucial. This is especially the case when considering accurate deviation bounds between a stochastic continuous-state model and its finite (reduced-order) abstraction. In this work, we introduce a coupling compensator to parameterize the set of relevant couplings and we give a comprehensive computational approach and analysis for linear stochastic systems. More precisely, we develop a computational method that characterizes the set of possible simulation relations and gives a trade-off between the error contributions on the systems output and deviations in the transition probability. We show the effect of this error trade-off on the guaranteed satisfaction probability for case studies where a formal specification is given as a temporal logic formula.

==> Efficient Similarity Quantification - Birgit/Commands.tex <==
\newcommand{\new}[1]{{\color{orange}#1}}

\newcommand{\CA}[1]{\mathcal{#1}}

\newcommand{\always}{\Box}
\newcommand{\eventually}{\Diamond}
\newcommand{\until}{\mathbin{\sf U}}
\newcommand{\release}{\mathbin{\sf R}}
\newcommand{\nex}{\mathord{\bigcirc}}

\newcommand{\My}{\mathcal{M}_\Y}
\newcommand{\M}{M}
\newcommand{\X}{\mathbb{X}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\Y}{\mathbb{Y}}

\newcommand{\Mh}{\hat{M}}
\newcommand{\Xh}{\hat{\mathbb{X}}}
\newcommand{\Uh}{\hat{\mathbb{U}}}
\newcommand{\Yh}{\hat{\mathbb{Y}}}

\renewcommand{\Pr}{\mathbb{P}}

\newcommand{\cdf}{\operatorname{cdf}}
\newcommand{\idf}{\operatorname{idf}}

\newcommand{\word}{\pmb{\pi} }
\newcommand{\letter}{\pi}
\newcommand{\FSA}{\mathcal A}
\newcommand{\Language}{\mathcal L}

\newcommand{\B}{\CA{B}}
\newcommand{\Bel}{{\mathbf {T}}}
\newcommand{\BelR}{{\mathbf {R}}}
\newcommand{\trunc}[2]{\operatorname{trunc}_{#1}\left(#2\right)}
\newcommand{\Lab}{\mathsf{L}}
\newcommand{\Labset}{\mathcal{L}}
\newcommand{\policy}{\mu}

\newcommand{\Wspace}{\mathbb{W}}
\newcommand{\Pw}{\mathbb{P}_w}

\newcommand{\AP}{\mathrm{AP}}

